Efficient Row-Level Lineage Leveraging Predicate Pushdown

Row-level lineage explains what input rows produce an output row through a data processing pipeline, having many applications like data debugging, auditing, data integration, etc. Prior work on lineage falls in two lines: eager lineage tracking and lazy lineage inference. Eager tracking integrates lineage tracing tightly into the operator implementation, enabling efficient customized tracking. However, this approach is intrusive, system-specific, and lacks adaptability. In contrast, lazy inference generates additional queries to compute lineage; it can be easily applied to any database, but the lineage query is usually slow. Furthermore, both approaches have limited coverage of the type of data processing pipeline supported due to operator-specific tracking or inference rules. In this work, we propose PredTrace, a lineage inference approach that achieves easy adaptation, low runtime overhead, efficient lineage querying, and high pipeline coverage. It achieves this by leveraging predicate pushdown: pushing a row-selection predicate that describes the target output down to source tables and querying the lineage by running the pushed-down predicate. PredTrace may require saving intermediate results when running the pipeline in order to compute the precise lineage. When this is not viable, it can still infer lineage but may return a superset. Compared to prior work, PredTrace achieves higher coverage on TPC-H queries as well as 70 sampled real-world data processing pipelines in which UDFs are widely used. It can infer lineage in seconds, outperforming prior lazy approaches by up to 10x.

==> approach.tex <==


\section{Model}

\subsection{Tuple Origins for Data Pipelines}
We adopt the definition of tuple provenance in relational operators in \cite{} to define the tuple provenance in data pipeline operators.

\begin{definition}[Data Lineage for Data Pipeline Operators]\label{def:lineage}
Let $Op$ be an operator in the data science pipeline over a set of input relations $T_1, \cdots, T_m$. Suppose a filter $F$ is applied on the operator output $T = Op(T_1, \cdots, T_m)$ to identify the pieces of information on $T$ that the data users want to explore. We define the origins of elements in $F(Op(T_1, \cdots, T_m))$ from input tables $T_1, \cdots, T_m$ to be the maximal subsets $T_1^*, \cdots, T_m^*$ such that:
\[(a) Op(T_1^*, \cdots, T_m^*) = F(Op(T_1, \cdots, T_m)) \]
\[(b) \forall T_i^*: \forall t^* \in T_i^*: \exists \hat{t} \text{ and an unique mapping } \mathcal{H}, s.t.,\] \[\hat{t} \in Op(T_1, \cdots, T_m) \text{ and } \mathcal{H}(t^*) = \hat{t}\]
\[(c) \forall T_i^*: \forall t^* \in T_i^*: F(Op(T_1^*, \cdots, \{t^*\}, \cdots, T_m^*)) \neq \emptyset \]


We define $Op^{-1}_{T_i}(F(Op(T_1, \cdots, T_m))) = T_i^*$ as the origins of the selected outputs $Op(T_1, \cdots, T_m)$ in the input table $T_i$. The set of origins of the $F(Op(T_1, \cdots, T_m)$ are $Op^{-1}_{<T_1, \cdots, T_m>}(F(Op(T_1, \cdots, T_m))) = \cup_{i = 1 }^m T_i^*$.
\end{definition}

In definition \ref{def:lineage}, requirement (a) requires that the origins $T_1^*, \cdots, T_m^*$ could exactly derives the output records in the desired set $F(Op(T_1, \cdots, T_m))$.  Requirement (b) shows that the records $\forall t^* \in T_i^*$ should be in the final result of the pipeline computations, i.e. there exists a record $\hat{t}$ in $F(Op(T_1, \cdots, T_m))$ and a unique mapping $\mathcal{H}$ that maps $t^*$ to one of the output record $\hat{t}$. For example, \yin{Develop a running example that (1) does have a join match (2) top n} \yin{Requirement (b) might not be strict enough but we can explain it using examples.}. Lastly, requirement (c) indicates that the all origin records $t^*$ will contribute to the final output in $F(Op(T_1, \cdots, T_m))$. 
%\yin{Do we want to keep the maximal subset requirement?}


\begin{example}
\yin{develop several examples about data lineage in data pipeline operators}
\end{example}


\begin{definition}[Data Lineage in Data Science Pipelines] Let $T$ be the output table of a data pipeline $P = \{Op_1, \cdots, Op_n\}$ on a set of input sources $S = \{S_1, \cdots, S_m\}$. A filter $F$
is applied to the output table $\mathcal{T}$ to identify tuples from the output for lineage exploration. The data origins of $F(T)$ is given by:
\[P^{-1}_{<S_1, \cdots, S_m>}(F(\mathcal{T})) = \cup_{i=1}^m S_i^* \]
where $S_1^*, \cdots, S_m^*$ are the subsets of input sources that $t^* \in S_i^*$ iff (1) $t^*$ contributes to the final result $T$. (2) there exists a record $\hat{t} \in T$ and a unique mapping $\mathcal{H}$ that $\mathcal{H}(t^*) = \hat{t}$. For all $t^* \in \cup_{i=1}^m S_i^*$,  we can derive exactly the output $T$ after the data processing of pipeline $P$.
\end{definition}



\begin{example}
\yin{add an example about data lineage in data pipelines,}
\end{example}


\subsection{Predicate Pushdown for Data Lineage}

\begin{problem}[Data Lineage by Predicate Pushdown]
Given a data pipeline $P= \{Op_1, \cdots, Op_n\}$ on the set of input sources $S = \{S_1, \cdots, S_m\}$ which generates the output $\mathcal{T}$, and a filter $F$ on $\mathcal{T}$ to identify the interested output pieces, find the set of input filters $G = \{G_1, \cdots, G_m\}$ on $S$ to get the origins from the input sources for the specified output pieces $F(\mathcal{T})$, i. e., for all $i \in m $, find the set of $G, s.t., G_i (S_i) = S_i^*,$ where,
\[P^{-1}_{<S_1, \cdots, S_m>}(F(\mathcal{T})) = \cup_{i=1}^m S_i^* \]
\end{problem}



\subsection{Lineage Superset Estimation}
Note that for predicate pushdown in data science pipelines, we aim to find the input filter $G$ that satisfies: $F(Op(T)) = Op(G(T))$. The lineage requirements proposed in Definition~\ref{def:lineage} cannot be guaranteed. Next we discuss the lineage superset and subsets given by predicate pushdown.


\begin{definition}[Lineage Superset]\label{def:superset}
Let $Op$ be an operator in the data science pipeline over the input relations $T_1, \cdots, T_m$. Suppose the set of interested output is given by a output filter $F$ as $F(Op(T_1, \cdots, T_m))$ and the predicate pushdown candidate $G$ gives a set of candidate origins $T_1^{sup}, \cdots, T_m^{sup}$, the candidate origins are lineage supersets of operator $Op$ when $T_1^{sup}, \cdots, T_m^{sup}$: satisfy the requirement (a) in data lineage definition (Definition \ref{def:lineage}) but does not satisfy requirement (b) and (c).
\end{definition}

\begin{example}[Data Lineage Supersets]
As shown in Figure~\ref{fig:superset}, the predicate pushdown gives an. 
\end{example}

\yin{Remove}
For some aggregate functions, finding the data lineage might over-approximates the set of data origins by a significant amount \cite{}. For example, for the min and max aggregation, the data lineage will returns all items belongs to this group as the origin to the final result. However, only the minimal and maximal value contributes to the min and max value. In these cases, finding the data lineage using predicate pushdown might be able to give a subset of the data lineage. Next, we formally define the lineage subset of data pipelines.

\begin{definition}[Lineage Subset]\label{def:subset}
Let $Op$ be an operator in the data science pipeline over the input relations $T_1, \cdots, T_m$. Suppose the set of interested output is given by a output filter $F$ as $F(Op(T_1, \cdots, T_m))$ and the predicate pushdown candidate $G$ gives a set of candidate origins $T_1^{sub}, \cdots, T_m^{sub}$, the candidate origins are lineage subsets of operator $Op$ when $T_1^{sup}, \cdots, T_m^{sup}$: satisfy the requirement (a) (b) (c) in data lineage definition (Definition \ref{def:lineage}) but does not satisfy the maximal subset requirement.

\end{definition}




\begin{table}[t]
\scriptsize{
  \caption{Lineage result compared with lineage tracking}
\vspace{-0.1in}
  \label{tab:superset}
  \begin{centering}
  \scalebox{1.2}{
  \begin{tabular}{l|l|l}
  \toprule
  Name & Equivalence& Example\\
  \midrule
  Filter & Equivalent&\\
  InnerJoin &  Superset& \begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{figures/F2.png}}
	\end{minipage}\\
  RowTransform & Equivalent&\\
  DropColumn & Equivalent&\\
  Reorder & Equivalent&\\
  GroupBy & Equivalent&\\
  Pivot &  Equivalent&\\
 CumAggr & Equivalent& \\
  %CumAggr & subset& \begin{minipage}[b]{0.3\columnwidth}
	% 	\centering
	% 	\raisebox{-.5\height}{\includegraphics[width=\linewidth]{figures/F1.png}}
	% \end{minipage}\\
  UnPivot &  Superset&\begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{figures/F6.png}}
	\end{minipage}\\
  RowExpand & Equivalent&\\
  TopK & Superset& \begin{minipage}[b]{0.3\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{figures/F3.png}}
	\end{minipage}\\
  GroupedMap & Superset& Give an example about topn\\
  RowIterPipeline & Superset&\\
  LeftOuterJoin & Superset&\\
  \bottomrule
\end{tabular}}
\end{centering}
}
\vspace{-0.1in}
\end{table}
\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.25]{figures/E1.png}
    \caption{Example of symbolic execution to determine when superset may arise.}
    \label{fig:my_label}
\end{figure*}



In Table \ref{tab:superset}, we summarize the lineage result given by predicate pushdown for the data science pipeline core operators proposed in \cite{}.





\yin{Reasons for superset to arise: }

\yin{Explain the reason for not guaranteeing the maximal set.}




\yin{Condition that needs sampling: (a) the pushed down G does not contain equality predicate on the join column. (b) inequivalence predicate only on the  id\_var, (c) topk with inequality on the value column.}




\section{Predicate Pushdown for Data Debugging}

\subsection{Predicate Pushdown in Data Science Pipeline Operators}


{\bf Show the input filter generation algorithm}

{\bf briefly talk about the predicate pushdown and verification workflow.}

\subsection{Lineage Superset Estimation}

To avoid over-estimation of the lineage set, we aim to detect when large superset might arise and take further steps to avoid returning large supersets. Next, we discuss how to estimate the size of the lineage supersets. 

As discussed in Definition \ref{def:superset}, lineage supersets arise when the candidate input filter $G$ gives a set of input origins that satisfy only the lineage requirement (a). Given a candidate set of data origins $\{G_1(T_1) = T_1', \cdots, G_m(T_m) = T_m'\}$ for an operator $Op$, we first check if the superset satisfy the lineage requirement (a), i.e., $Op(T_1', \cdots, T_m') = F(Op(T_1, \cdots, T_m))$. If satisfies, we next check whether there exists a one-to-one match of the input to the output table. To determine the size of the in

\begin{example}
\yin{Example of }
\end{example}

(1) 

The set of passes input filter $G$ but does not satisfy the 


{\bf determine when superset might arise}




\begin{algorithm}[h]
\algblock[TryCatchFinally]{try}{endtry}
\algcblock[TryCatchFinally]{TryCatchFinally}{finally}{endtry}
\algcblockdefx[TryCatchFinally]{TryCatchFinally}{catch}{endtry}
	[1]{\textbf{catch} #1}
	{\textbf{end try}}
\begin{algorithmic}[1]
\caption{Input Sampling}
\label{algo:sample}
\Procedure{InputSampling}{$\{T_1, \cdots, T_m\}$}
\State{\it Set the default Sampler $S_i$ on each input $T_i$ relation as the uniform sampler.}
\For {$op_i$ $\in$ pipeline $P$}
    \If {$op_i$ is a join operator}
        \State {\it Universe Sampler $\rightarrow S_k, S_j$, where $T_k, T_j \in \{T_1, \cdots, T_m\}$ are the source input of the join relations.}    
                % \State {\it Set a universe sampler on input table $T_i$ and $T_j$, where the groupby columns originate.}
    \EndIf
% satisfy distinct first
    \If {$op_i$ is a groupby or pivot operator}
        \State {\it Distinct Sampler $\rightarrow S_k,$, where $T_k \in \{T_1, \cdots, T_m\}$ is the input table where the groupby columns originate.}    
        % \State {\it Set a distinct sampler on input table $T_k$, where the groupby columns originate.}
    \EndIf
\EndFor 
\For {$T_i \in \{T_1, \cdots, T_m\}$}
        \State {\it Use $S_i$ with parameters $p, \sigma$ to get a set of samples from $T_i$ as $T_{si}$.} 
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-0.1in}

\yin{Need better illustration of sampling parameters}

\begin{algorithm}[h]
\algblock[TryCatchFinally]{try}{endtry}
\algcblock[TryCatchFinally]{TryCatchFinally}{finally}{endtry}
\algcblockdefx[TryCatchFinally]{TryCatchFinally}{catch}{endtry}
	[1]{\textbf{catch} #1}
	{\textbf{end try}}
\begin{algorithmic}[1]
\caption{Superset estimation}
\label{algo:superset}
\Procedure{SupersetEstimation}{$Op_i, G,  P, t, (T_{s1}, \cdots, T_{sm})$}

\State {Execute the data pipeline $P$ on $(T_{s1}, \cdots, T_{sm})$ until the operator $Op_{i-1}$ to get sampled input $T'$ of operator $Op_i$.}

\State{$s1 \leftarrow G(T')$} \Comment{Get the number of records pass filter $G$}
\State{$s2 $} \Comment{Get the number of records are not filtered out in the operator $Op_i$}
\If{$(s1 - s2) > t$}
\Return {True}
\EndIf



\EndProcedure
\end{algorithmic}
\end{algorithm}
\vspace{-0.1in}



\begin{algorithm}[h]
\algblock[TryCatchFinally]{try}{endtry}
\algcblock[TryCatchFinally]{TryCatchFinally}{finally}{endtry}
\algcblockdefx[TryCatchFinally]{TryCatchFinally}{catch}{endtry}
	[1]{\textbf{catch} #1}
	{\textbf{end try}}
\begin{algorithmic}[1]
\caption{Data Lineage with Superset Estimation}
\label{algo:lineage}
\Procedure{Lineage}{$\{T_1, \cdots, T_m\}$, $P$, $F$}
\State $T_{s1}, \cdots, T_{sm} \leftarrow$ {\sc InputSampling($\{T_1, \cdots, T_m\}$)}

\For {$op_i$ $\in$ pipeline $P$}
    \State {$G_i\leftarrow$ {\sc CandidateGen($F_i, op_i$)}
    \If {$op_i \in$ [InnerJoin, UnPivot, TopK, LeftOuterJoin, GroupedMap, RowIterPipeline]} \yin{Some condition satisfied}
    \State {Flag $\leftarrow$ {\sc SupersetEstimation($op_i, G_i, (T_{s1}, \cdots, T_{sm}) $)}
    \While{Flag = True}
        \If {$F_i' \leftarrow$ {\sc InputFilterRewrite($F$)}, $F_i' != F_i$}
        \State {$G_i' \leftarrow$ {\sc CandidateGen($F_i', op_i$)}
        \Else
        \State {$G_i' \leftarrow$ {\sc Snapshot($F_i', op_i$)}
        \EndIf
    \State {Flag $\leftarrow$ {\sc SupersetEstimation($op_i, G_i', (T_{s1}, \cdots, T_{sm})$)}
    \EndWhile    
    \EndIf
    \State {$F_{i+1} = G_i$}
\EndFor


\EndProcedure

\end{algorithmic}
\end{algorithm}




\paragraph{Universe Sampler}
\paragraph{Distinct Sampler}

\paragraph{Superset Estimation with Samplers}
\yin{talk about when to }



\subsection{Output Filter Rewrite}
{\bf rewrite input filter to get equivalent }

\subsection{Snapshot}


{\bf snapshot}


\subsection{Data Debugging in Data Science Pipelines}


{\bf talk about the condition}











\yin{Prove why row transformation could also satisfy the requirement b) and (c).}

\yin{Show the reason how superset could arise for aggregation pipeline. }

\yin{Show the reason how superset could }


(1) 
(2)
(3) 


% decide when superset might happen
% (1) returns a superset G


% (2) operators that would gives a superset:
% (1)Some operators modified the output filter F.
% (2) The output filter F causes superset when it is pushdown to an operator $Op$.



% (2) How to determine when a superset would arise?
% It does not satisfy the lineage requirement:
% $$\forall T_i^*: \forall t^* \in T_i^*: Op(T_1^*, \cdots \{t^*\}, \cdots T_m^*) = \emptyset $$
% where $T_i^*$ are the subsets from the input table $T_i$.

% method:
% \begin{itemize}
%     \item Given a symbolic table T. Execute the input filter $G$ on T to get $T^*$. 
%     \item Check for each $t^* \in T^*$: Execute $Op(t^*)$, get $F(Op(t^*))$.
%     \item Check if $F(Op(t^*)) = \emptyset$. If yes, then it means we get a superset.
% \end{itemize}

% Example:






{\bf When the superset is large, take a snapshot.}



==> model.tex <==
\vspace{-2mm}
\section{Data lineage inference leveraging predicate pushdown}
\label{sec:model}
%In this section, we explore the theoretical foundation to use predicate pushdown to compute data lineage, and discuss how 

In this section, we illustrate the lineage model and the theoretical foundation of computing lineage using predicate pushdown.
%, and show how to leverage an existing pushdown module. 
%We start with a single operator, and extend to a data pipeline.

%\subsection{Single Operator}

\vspace{-2mm}
\subsection{Lineage model}
\label{sec:model-define}
We extend the lineage model of prior work~\cite{ikeda2013logical} to include non-relational operators and UDFs.

\vspace{-2mm}
\subsubsection{Single operator} 
We start with a single operator. Let $Op$ be an operator over tables $T$ which produces an output table $T_{out}$ (i.e., $T_{out}=Op(T)$). {\bf Given a tuple $t_o$ from $T_{out}$, the lineage of $t_o$ is a minimal subset of $T$ (denoted as $T^*$) such that $Op(T^*)=\{t_o\}$. In other words, $t_o$'s lineage is a minimal subset of $Op$'s inputs that can produce the output $t_o$.} When the minimal subset is not unique, the lineage is the union of all minimal subsets. 

% \revised{
% While \tool guarantees to return the exact lineage when intermediate result can be saved, it might return a lineage superset without saving intermediate result.
% We define {\bf lineage superset}, $T^\supset$, as a superset of the minimal $T^*$ that can produce $t_o$, i.e., $T^\supset\supset T^*$ and $Op(T^\supset)\supseteq\{t_o\}$. 
% }

% \vspace{-2mm}
\subsubsection{Data pipeline}
The definition also applies to a data pipeline. Because the lineage on a single operator is transitive, the lineage of a data pipeline can be computed operator-by-operator backward following the dataflow graph. 
%For lineage superset, which is not transitive, the lineage 

% \vspace{-2mm}
\subsubsection{Examples}
\label{sec:model-example}
We provide a few examples to explain how the lineage model applies to non-trivial operators and UDFs.

\begin{asparaitem}
\item {\it Example 1.} Semi-join operator, e.g., SELECT * FROM {\dbtable R} EXISTS (SELECT * FROM \dbtable{S} WHERE \dbfield{R.a}=\dbfield{S.a}). Given an output $t_o$, the lineage of the outer table {\dbtable R} is precisely $t_o$ itself; for inner table {\dbtable S}, the minimum subset is one joinable row with $t_o$. If more than one row is joinable, the lineage is the union of all joinable rows.

\item {\it Example 2.} Anti-join operator, e.g., SELECT * FROM \dbtable{R} NOT EXISTS (SELECT * FROM \dbtable{S} WHERE \dbfield{R.a}=\dbfield{S.a}). Given a $t_o$, the lineage from table {\dbtable R} is $t_o$ itself. For table \dbtable{S}, the lineage is an empty set, as when \dbtable{R} contains only $t_o$ and no other rows, the anti-join has no effect when computing $Op(T^*)$ and hence can be an empty set.
% From table {\dbtable S} the lineage is an empty set, as when {\dbtable R} includes only $t_o$ and no other rows, the anti-join has no effect when computing $Op(T^*)$ and hence can be an empty set.


\item {\it Example 3.} UD-Aggregate, e.g., SELECT * FROM \dbtable{R} GROUP BY \dbtable{a} MAX(IF \dbtable{x} IS NOT NULL \dbtable{x} ELSE \dbtable{y*z})
%\footnote{This query does not follow standard SQL syntax. We use this SQL-like expression only for illustration purposes.} 
where the user-defined aggregation selects the max of {\dbfield x} or {\dbfield y}*{\dbfield z} depending on whether \dbtable{x} is NULL. Given a $t_o$, the lineage contains only the rows belonging to group $t_o.a$ whose {\dbfield x} value is the same as $t_o.\max$ or {\dbfield x} is NULL while {\dbfield y}*{\dbfield z} equals to $t_o.${\dbfield max}.


\item {\it Example 4.} UD-SubQuery, e.g., SELECT R.a AS a, (IF (exists (SELECT * FROM {\dbtable S} WHERE {\dbtable S.a}={\dbtable R.a}), 0, {\dbtable R.v})) AS {\dbtable v} FROM {\dbtable R}. For each row in table {\dbtable R}, this query returns 0 as field {\dbfield v} if there exists any row from table {\dbtable S} that matches the value of {\dbfield R.a}.
Otherwise, field {\dbfield v} is set to the value from {\dbfield R.v}. Giving a $t_o$, it might be computed from one of the two sources (i.e., two potential lineage sets): 1) the row from {\dbtable R} with the same value as $t_o$ when the IF condition is evaluated as False, or 2) the rows {\dbtable S} whose field {\dbfield S.a} matches $t_o$.{\dbfield a} when the IF condition is evaluated as True.


\end{asparaitem}

% \revised{
% We also define {\bf lineage superset}, $T^\supset$, which is a superset of the minimal $T^*$ that can produce $t_o$, i.e., $T^\supset\supset T^*$ and $Op(T^\supset)\supseteq\{t_o\}$.
% }


%we can obtain $t_o$'s lineage at intermediate result $T_{i-1}$ by the single-operator's lineage model, denoted as $T^*_{i-1}$. Then, we take the union of every tuple of $T^*_{i-1}$'s lineage at $T_{i-2}$ as $T^*_{i-2}$, and so on, until we reach the pipeline's input $T_0$ and obtain $T^*_0$.

\vspace{-2mm}
\subsection{Lineage inference using predicate pushdown} \label{sec:pushdown}
% \yin{Can we say what if pushing down $F^{row}$ and $F$ fails very briefly here to give an overview? Discussing them in the paragraphs seems a little ad hoc.}
\label{sec:lineage-pushdown}
% \label{sec:pipeline}
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.4]{figures/5.pdf}
%     \caption{\textnormal{Lineage model and inference using predicate pushdown.}}
%     \vspace{-4mm}
%     \label{fig:lineage-pushdown}
%     \vspace{-2mm}
% \end{figure}


%\cong{TODO: add column "contain UDF", default Grow explained, and pushdown $\emptyset$.}
\begin{table*}
  \caption{\textnormal{Core operators of \tool, what UDF is supported, and the default $G^{row}$ used if pushing down $F^{row}$ fails.}}
\scriptsize{
\vspace{-0.15in}
  \label{tab:basic-ops}
  \begin{centering}
  \scalebox{1.17}{
  \setlength{\tabcolsep}{1.5pt} % Adjust the column spacing here
  \begin{tabular}{lllll}
  \toprule
  {\bf Operator} & {\bf Description} & {\bf embedded UDF supported} & {\bf default $G^{row}$ if pushdown fails} & {\bf default $G^{row}$ explained} \\
  \midrule
  Filter & selection in SQL & UD-selection predicate & $F^{row}\wedge$ filter-predicate & Select the same row as $t_o$\\
  \hline
  InnerJoin & innerjoin in SQL & UD-join predicate & \makecell[l]{$col_{l_1} == v_{l_1} \wedge \cdots$ (left)\\ $col_{r_1} == v_{r_1} \wedge \cdots$ (right)} & \makecell[l]{Select the rows from left/right table which\\produce $t_o$ after joined} \\
  \hline
  RowTransform &  row/scalar transform & UD-transform function & $f_1(col_1,col_2\cdots) == v_1\wedge\cdots$ & \makecell[l]{Select the row that transformed\\into the values of $t_o$}  \\
  \hline
  DropColumn &  projection in SQL  & NA & $F^{row}$ & Select the same row as $t_o$   \\
  \hline
  Reorder/TopK & order-by (LIMIT N) in SQL & UD-compare function  & $F^{row}$ & Select the same row as $t_o$  \\
  \hline
  Union/Intersect & union/intersection in SQL & NA & $F^{row}$ & Select the same row as $t_o$ \\
  \hline
  GroupBy & groupby in SQL & UD-aggregation & $col_{group} == v_i$ & Select the entire group\\
  \hline
  Pivot &  pivot operator & UD-aggregation & $col_{index} == v_i\wedge$ & Select the entire index group  \\
  \hline
  UnPivot  & unpivot operator & NA &  $col_{index}==v_1\wedge col_{v_2}==v_3$ & Select the entire index group  \\
  \hline
  RowExpand &  1-to-k transformation & UD-expand function & \makecell[l]{$(f_1(col_1,col_2,\cdots)[0] == v_1\vee$\\$f_1(col_1,col_2,\cdots)[1] == v_1) \wedge \cdots$} & \makecell[l]{Select the row if any row from its\\expanded K-row output is the same as $t_o$} \\
  \hline
  LeftOuterJoin & left/right outer join & UD-join predicate &\makecell[l]{$col_{l_1} == v_{l_1} \wedge \cdots$ (left)\\ $col_{r_1} == v_{r_1} \wedge \cdots$ or $False$ (right)} & \makecell[l]{Select the row matching $t_o$ from left table,\\the joined row from right table if \\right column values from $t_o$ are not NULL,\\o.w. select empty set from right table}\\
  \hline
  WindowOp & rolling/diff like ops & NA &  $col_{index}\in [i,i+$window\_size$]$ & Select the entire window used to produce $t_o$\\
\midrule
  GroupedMap & \makecell[l]{transform grouped sub-\\tables with a subquery} &  \makecell[l]{Subquery defined in\\ core operators} & $col_{group} == v_i$ & Select the entire group \\
    \hline
  SemiJoin & EXIST/IN subquery & \makecell[l]{Subquery defined using\\core operators} & \makecell[l]{$F^{row}$ (outer)\\push $True$ to inner query, (inner)\\replace correlated column $col_i$ with $v_i$} & \makecell[l]{Select same $t_o$ from outer table;\\select all rows returned by inner query with\\specific correlated column value $v_i$ from $t_o$} \\
  \hline
  AntiJoin & NOT EXIST subquery &  \makecell[l]{Subquery defined using\\core operators} & \makecell[l]{$F^{row}$ (outer)\\ push $False$ to inner query} & \makecell[l]{Select same $t_o$ from outer table\\empty set from inner query result}  \\
    \hline
  SubQuery & \makecell[l]{For each row, the subquery\\computes with other tables\\to return a value $v$} & \makecell[l]{Subquery defined using\\core operators} & \makecell[l]{$F^{row}$ (outer)\\push $col_v==v$ to inner query, (inner)\\replace correlated column $col_i$ with $v_i$} & \makecell[l]{Select same $t_o$ from outer table\\all rows used to produce value $v$ from inner table} \\
  \bottomrule
\end{tabular}}
\end{centering}
}
 \vspace{-0.1in}
\end{table*}

\subsubsection{Single operator} 
We first show how to leverage predicate pushdown to infer lineage for a single operator.
We define {\it row-selection predicate} $F^{row}$, constructed from a concrete row $t$, as $(col_1==v_1\wedge col_2==v_2\wedge\cdots)$ where $v_1,v_2,\cdots$ are corresponding values from $t$. In other words, $F^{row}(Op(T))=\{t\}$ under set semantic. 
Given a $t_o$ from the output, we construct $F^{row}$ and push it through $Op$. If the pushed $G^{row}$ is the most selective predicate\footnote{There is no need to consult cardinality estimator to decide selectivity, as $G^{row}$ is a conjunction of equal comparisons, therefore predicate with the most conjunctions is the most selective.} that ensures $Op(G^{row}(T))=F^{row}(Op(T))$, $G^{row}$ selects the precise lineage.

% \footnote{It holds on any $T$ when $F^{row}(Op(T))\neq\emptyset$. We encode this non-empty output as an assumption and send it to MagicPush.}


We rely on an external pushdown module like MagicPush \cite{predicate-pushdown}, which often returns a most selective $G^{row}$.
To ensure the successful pushdown of row-selection predicates, \tool provides a set of default $G^{row}$ as listed and explained in Table~\ref{tab:basic-ops}, for cases where the module fails. Usually, the default $G^{row}$ is the same as the $G^{row}$ obtained through predicate pushdown.
 However, there are scenarios where the default $G^{row}$ may differ, returning a lineage superset for certain UDFs.
For example, in a groupby operation with max aggregation, the precise lineage includes only the row with the maximum value, not the entire group.


% , such as when pushing down $F^{row}$ through a filter operator. 
% If the pushdown module fails to return a $G^{row}$ for a $F^{row}$, \tool uses a default $G^{row}$ as listed and explained in Table~\ref{tab:basic-ops}. This default $G^{row}$ is customized for each category of the operator, and often it is the same as the $G^{row}$ obtained through predicate pushdown.

%, albeit not guaranteed. Therefore \tool includes a procedure to examine whether the returned $G^{row}$ is indeed selecting the exact lineage (we omit it due to space limit but present it in~\cite{techreport}). 


In our experiment, MagicPush is always capable of pushing down $F^{row}$ successfully, and the corresponding $G^{row}$ is the most selective predicate returning the minimal lineage.
Therefore, \tool rarely needs to fall back on the default $G^{row}$ in practice.
% for UDFs like groupby-max.
%, being capable of finding the minimal lineage, which is not achieved by prior work. 

\vspace{-2mm}
\subsubsection{Data pipeline}
Assume every intermediate result is stored, using predicate pushdown to obtain lineage is straightforward: at each $Op_i$, we push $F^{row}_i$ to obtain $G^{row}_i$, run $G^{row}_i$ on $Op_i$'s input which is materialized, obtain concrete rows and represent them using $F^{row}_{i-1}$, and continue to push $F^{row}_{i-1}$ to $Op_{i-1}$.


However, saving every intermediate result is too costly. We may skip saving $Op_{i-1}$'s output and push $G^{row}_i$ instead of the row-selection $F^{row}_{i-1}$ through $Op_{i-1}$. Consequently, at $Op_i$, we may push down a non-row-selection predicate $F_i$ and obtain another non-row-selection predicate $G_i$. \tool verifies whether this $G_i$ yields the same outcome as if we push down $F^{row}_i$, as demonstrated later in Section~\ref{sec:smt-minimal}. 
% \yin{TODO}
Additionally, the predicate pushdown module may fail when attempting to push the non-row-selection predicate $F_i$. If either failure occurs, i.e., $G_i$ returns a different result than $G^{row}_i$ or pushing $F_i$ fails, we fall back to save the intermediate result.

% Moreover, since $F_i$ is a non-row-selection predicate, attempting to push it down may fail, and we lack a default solution for such cases. If either failure happens, i.e., $G_i$ returns a different result than $G^{row}_i$ or pushing $F_i$ fails, we fall back to save the intermediate result.

%Because $F^{row}_{i-1}$ is concretized from running $G^{row}_i$ on the intermediate result, they are equivalent on any specific table instance, and pushing $G^{row}_i$ have the same effect. 
%Unfortunately, $G^{row}_i$ is no longer a row-selection predicate,



Note that, when $Op_i$'s input is saved, running $F_i$ on the result may yield multiple rows. However, since we can infer for each row individually, we still push down a parameterized single-row-selection $F^{row}_i$=$col_1=v_1\wedge\cdots$ to simplify the pushdown process. 
When the final $PLineage$ at the source table involves only variables from one intermediate result with N rows, we disjunct these N instances for $PLineage$, where each instance replaces variables $v_1, \cdots$ with the column values of one row. 
The disjunction may become large if the $PLineage$ involves variables from multiple intermediate results as we need to disjunct all combinations. However, such a scenario rarely happens due to our optimization in Section~\ref{sec:opt}, which tends to save one intermediate result at a later stage in the pipeline rather than multiple results. 


%\yin{Hi Cong, can you double-check if the above is correct?}
% When the final $PLineage$ at the source table involves only variables from one intermediate result, we disjunct N instances of this predicate if the intermediate result contains N rows, each instance replacing $v_1$ with one row's value. 
%\cong{TODO: how to concretize intermediate result.}

% \revised{
% Because $G^{row}_i$ is no longer a row-selection predicate, we need to check whether pushing it down selects the same rows on $Op_{i-1}$'s input as if we push down row-selection predicate $F^{row}_{i-1}$.} 
% If yes, we skip this intermediate result, otherwise we fall back to saving it.

\vspace{-2mm}
\subsubsection{Examples}
We revisit the examples in Section~\ref{sec:model-example} and see how pushing down $F^{row}$ can select the exact lineage.

\begin{asparaitem}
\item {\it Example 1.} When pushing down $F^{row}$ through the semi-join, the most selective predicate on table \dbtable{R} is the same $F^{row}$ selecting exactly $t_o$, while on table \dbtable{S} is {\dbfield S.a}=$t_o$.{\dbfield a} that selects joinable rows. 

\item {\it Example 2.} Pushing down $F^{row}$ to table {\dbtable R} yields the same $F^{row}$, while to table {\dbtable S}, the predicate $G^{row(R)}$ is \texttt{False}. These are the most selective predicate that ensures $F^{row}(Op(T_R, T_S))=$\\$Op(G^{row(R)}(T_R),G^{row(S)}(T_S))$.


\item {\it Example 3.} Pushing down $F^{row}$=({\dbfield a}=$v_a\wedge${\dbfield max}=$v_m$) through the groupby with a user-defined aggregation would return $G^{row}$ as follow: {\dbfield a}=$v_a\wedge$(({\dbfield x}$\neq$ NULL$\wedge${\dbfield x}=$v_m$)$\vee$({\dbfield x}=NULL$\wedge${\dbfield y}*{\dbfield z}=$v_m$)). This $G^{row}$ selects the exact lineage rows as described in Section~\ref{sec:model-example}.


\item {\it Example 4.} This example includes a subpipeline, and we will discuss how pushdown works operator-by-operator. Pushing down $F^{row}$ to table {\dbtable R} returns the same $F^{row}$, and pushing it through the IF condition to table {\dbtable S} yields a predicate {\dbfield S.a}=$t_o$.a. When the branch condition evaluates to False, then $F^{row}$ selects precisely the output $t_o$ while no row matches the predicate on {\dbfield S}; when the branch condition evaluates to True, the matching rows from {\dbfield S} is selected by the pushed predicate. So in either case, the pushed predicate can return $t_o$'s lineage.

%-THEN-ELSE statement yields a \texttt{True} value for the branch condition, and obtain a {\dbfield v}=$t_o$.{\dbfield v} predicate through the statement. Pushing the \texttt{True} predicate further through the \textit{exist} subquery returns predicate {\dbfield S.a}=$t_o$.a, selecting all {\dbtable S} rows with matching value on {\dbfield a}. At table {\dbfield R}, a conjunction of {\dbfield a}=$t_o$.{\dbfield a} (the remaining of $F^{row}$) and {\dbfield v}=$t_o$.{\dbfield v} (from the IF-THEN-ELSE) is formed, yielding the final predicate on {\dbfield R}, returning the precise lineage. 
% }

% \revised{
% If $t_o$.{\dbfield v} evaluates to -1, then pushing down $F^{row}$ through the IF-THEN-ELSE statement yields a \texttt{False} value for the branch condition, which leads to an empty set on the {\dbfield S} table. Only the remaining of $F^{row}$, (i.e. {\dbfield a}=$t_o$.{\dbfield a}), is pushed to table {\dbfield R}. 
% }
\end{asparaitem}

\vspace{-1mm}
\subsection{Verification for non-row-selection predicate}
\label{sec:verification-nonrowsel}

%\ifTechReport
\label{sec:smt-minimal}
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{figures/counter-ex.png}
    \vspace{-8mm}
    \caption{\textnormal{Verification for non-row-selection predicate.}}
    \vspace{-5mm}
    \label{fig:counter-ex-minimal}
\end{figure}

Next, we illustrate how \tool decides whether pushing down a non-row-selection predicate can return an equivalent result as pushing down a row-selection predicate. Briefly, given an arbitrary predicate $F$, and its corresponding pushdown predicate $G$, we can construct a row-selection predicate $F^{row}$ from $F$, push it down as $G^{row}$, and prove that $G$ is equivalent to $G^{row}$. 

We illustrate using the SubQuery operator ($Op_4$) in Q4, where \tool tries to push down a non-row-selection predicate $F=$ \dbfield{o\_orderpriority}==$v_g$. First, we construct symbolic tables, each with one tuple where cell values are represented using symbols like $v_1,v_2,v_3$, as shown in Figure \ref{fig:counter-ex-minimal}(1). \tool first pushes down a non-row-selection predicate $F$, \dbfield{o\_orderkey}==$v_g$. It symbolically runs the obtained $G_o$ on \dbtable{orders} table, with the result shown in Figure \ref{fig:counter-ex-minimal}(2). We use a {\it row-exist} expression to indicate the condition of the row to survive the filter, e.g., $v_2==v_g$. It also runs the pushed $G_l$=\texttt{True} on the \dbtable{lineitem} table. 

\tool then constructs a $F^{row}$, pushes it down to obtain $G^{row}_o$ and $G^{row}_l$, and similarly runs them on their corresponding table, with the results shown in Figure \ref{fig:counter-ex-minimal}(3).

Finally, \tool verifies whether $G$ is equivalent to $G^{row}$ when $F^{row}$ is equivalent to $F$. This is essentially verifying the corresponding result tables, particularly these {\it row-exist} expressions, are equivalent regardless of the values of $v_{1,2,3}$. In this case, the verification fails as $G_l$ is not equivalent to $G^{row}_l$ (i.e., \texttt{True} is not equivalent to $v_3==v_k$). Therefore, we cannot use $G$ but need to fall back to saving the output of $Op_4$ and push down $F^{row}$. Because the equivalence of two predicates is in first-order logic, the verification using an SMT solver is sound and complete.
%\fi

\vspace{-2mm}
\subsection{Lineage superset} \label{sec:relaxed-model}
% \yin{This symbol is a little confusing, is it $T^{*\supseteq}$? It is a superset of $T^*$ and a subset of $T$. }\cong{Sounds good, can you change all the symbols to make it $T^{*\supseteq}$?}
% \yin{I find the term "lineage superset" somewhat unclear in certain contexts. For example, in this section, lineage superset means $Op(T^{*\subseteq})\supseteq \{t_o\}$. But in Section 3.3, we use "superset" to describe relationships like $T^{*\subseteq} \supseteq T^*$. I agree it is beneficial to use the first term to define both cases collectively. We might need to clarify in this section that the following three operators are partial reasons for lineage superset. Currently, the description suggests they are the sole causes.}\cong{I updated the definition. Does it look better?}
For three operators, {\it Unpivot}, {\it RowExpand}, and {\it WindowOp}, the lineage model in Section~\ref{sec:model-define} is not applicable because no subset of the input can precisely produce ${t_o}$. For instance, each input row transforms into multiple output rows through {\it RowExpand}, thereby making it impossible for a lineage row to produce the output $t_o$ exclusively. 
Therefore, we have to relax the lineage model for these operators. We define {\bf lineage superset $T^{*\supseteq}$ as a subset of the input $T$ and a superset of the precise lineage (i.e., $T^*\subseteq T^{*\supseteq} \subseteq T$) which is able to produce the target output row $t_o$ (i.e., $Op(T^{*\supseteq})\supseteq \{t_o\}$}). We want to emphasize that not every superset of $T^*$ is a valid lineage superset; only those that can produce the target output are valid. 
% For non-monotonic operators, a superset of the input may not guarantee the query result includes the output, making such supersets invalid. 
Additionally, such a superset is not unique and can be as large as the entire set $T$.
% This may be non-trivial to validate for non-monotonic operators, in which a superset of input may lead to a subset of output. Also note that such superset is not unique, and can be potentially as large as the entire $T$.

Compared to the precise lineage model in Section~\ref{sec:model-define}, having $\supseteq$ rather than $=$ in the superset model makes it no longer transitive: computing the superset operator-by-operator may not yield a valid lineage superset for the entire pipeline that guarantees the production of the target output $t_o$.
This is because running $Op_{i-1}$ on a lineage superset (i.e., $Op_{i-1}(T_{i-1}^{*\supseteq})$) returns an output including more rows than the precise lineage $T^*_i$ for the next operator $Op_i$. When $Op_i$ is a {\it non-monotonic} operator, computing $Op_i$ on a superset of the precise lineage cannot guarantee to produce the expected target output.

% \yin{Maybe not talk about predicates here.}
% \yin{Typo? $G_i$ instead of $G_{i+1}$.}\cong{updated, please double check} 

This issue can be resolved by leveraging predicates. 
As described in Section~\ref{sec:lineage-pushdown}, at each operator, we obtain a predicate through pushdown that guarantees to produce the target output, e.g., $G_i$ which ensures $G_i(Op_{i-1}(T_{i-1}))=\{t_o\}_{i}$ on any table $T_i$. This means that we can use $G_i$ to reduce any superset (e.g., $Op_{i-1}(T_{i-1}^{*\supseteq})$) to be a valid lineage superset, i.e., ensuring to produce the target $\{t_o\}_{i}$. 

% \yin{It is unclear to me why the pushed-down predicate $G_i$ is applied to the output of $Op_i$ in the formula.} 

% Based on the above intuition, {\bf we ensure that any lineage superset obtained through predicate pushdown is able to produce the target output}. The only change when producing the target output using the lineage superset lies in applying $G_{i+1}$ on the output of $Op_i$ before using it to compute the next $Op_{i+1}$. 

\vspace{-4mm}
\subsection{Lineage superset using predicate pushdown} \label{sec:superset_pushdown}

If lineage superset is allowed, we no longer need to save any intermediate result. When pushing down a row-selection predicate $F_i$ through a single operator $Op_i$, we obtain a predicate through MagicPush that guarantees $F_i(Op_i(G_i(T_i)))=F_i(Op_i(T_i))$ (i.e., the pushdown that allows $G_i(Op_i(T_i))$ to return a superset), and then continues to push the $G_i$. The lineage superset is selected by $G_i$, i.e., $T_i^{*\supseteq}=G_i(T_i)$. 

% \yin{i.e. contains all lineage rows and guarantees the output of $t_o$?}
We now prove that $G_i(T_i)$ is a valid lineage superset. Specifically, we want to demonstrate, for each $i$, (1) $G_i(T_i)\supseteq T_i^*$ (where $T_i^*$ is the precise lineage), and (2) $Op_i(G_i(T_i))\supseteq T_{i+1}^*$ (where $T_{i+1}^*$ is the precise lineage from $T_{i+1}$, which is the target output at operator $Op_i$). We prove this by induction. Assuming $G_{i+1}(T_{i+1})\supseteq T_{i+1}^*$ holds, (2) is satisfied as MagicPush ensures $Op_i(G_i(T_i))\supseteq F_i(T_{i+1}) = G_{i+1}(T_{i+1})\supseteq T_{i+1}^*$. 
Given that $G_{i+1}(T_{i+1})\supseteq T_{i+1}^*$ holds by assumption, (1) is also trivially satisfied as $T_i^*$ is the {\it minimum} subset that can produce the target output $T_{i+1}^*$, then any other subset of $T_i$ producing $T_{i+1}^*$ would be a superset of $T_i^*$. 

% \yin{For ``Given that $F_i(T_{i+1}) = G_{i+1}(T_{i+1})\supseteq T_{i+1}^*$ holds by assumption'', I don't understand how this assumption is used for inducing the second part of the conclusion (the connection is not very clear to me). }
% \yin{I am also not sure if the induction is correctly stated. Now we are trying to say assume (1) holds and (2) is correct and vice versa. Should we instead say something like i holds and i+1 also holds instead for induction?}
% While $F_i(T_{i+1})=G_{i+1}(T_{i+1})\supseteq T_{i+1}^*$ holds by assumption, (1) is trivially satisfied as $T_i^*$ is the {\it minimum} subset that can produce the target output $T_{i+1}^*$, then any other subset producing $T_{i+1}^*$ would be a superset of $T_i^*$. \yin{?}

% We now prove that $G_i(T_i)$ is a valid lineage superset. That is, we want to prove that (1) at each $i$, $G_i(T_i)\supseteq T_i^*$ (where $T_i^*$ is the precise lineage), and (2) $Op_i(G_i(T_i))\supseteq T_{i+1}^*$ (where $T_{i+1}^*$, the precise lineage from $T_{i+1}$, is the target output at operator $Op_i$). We prove this inductively. Assuming $G_{i+1}(T_{i+1})\supseteq T_{i+1}^*$ holds, (2) is satisfied as MagicPush ensures $Op_i(G_i(T_i))\supseteq F_i(T_{i+1})$, while $F_i(T_{i+1})=G_{i+1}(T_{i+1})\supseteq T_{i+1}^*$ holds by assumption. Then (1) trivially satisfies as $T_i^*$ is the {\it minimum} subset that can produce the target output $T_{i+1}^*$, then any other subset producing $T_{i+1}^*$ would be a superset of $T_i^*$. 

While we rely on MagicPush to return the most selective $G_i$, the superset can still be too large to be useful (e.g., including the entire {\dbtable lineitem} table in Q4). In Section~\ref{sec:minimize_superset}, we describe an algorithm to reduce the superset, making it, in many cases, as small as the precise lineage.
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.48]{figures/symbols.png}
%     \vspace{-10mm}
%     \caption{\textnormal{Illustration of symbols used in Section~\ref{sec:relaxed-model}. \yin{TO be updated}}}
%     \label{fig:proof-symbols}
%     \vspace{-2mm}
% \end{figure}







% $Op_i,Op_{i+1}$, $T_i,T_{i+1},T_{i+2}$, 
% $T_i^*,T_{i+1}^*$
% $F_{i+1}$ runs on $T_{i+2}$, returns a superset $T_{i+1}$
% returns $G_{i+1}$, $F_{i+1}(Op_{i+1}(G_{i+1}(T))=F_{i+1}(Op_{i+1}(T))$


% $G_{i+1}(Op_{i+1}(T_{i+1}))$ include $\{t_o\}_{i+1}$
% verify $G_i(T_i)$ can produce 

%Formally speaking,  the relaxed lineage model is transitive. We prove this property as follow. Assuming $F_i$ is a filter that returns a superset of the precise lineage $T_{i+1}^*$, we want to show that pushing down $F_i$ through $G_i$





%This relaxed lineage model, with the help of predicate, guarantees that we are able to produce the target output using a superset of the minimum lineage rows.  


%so computing the pipeline lineage using this relaxed model does not guarantee the production of the output $t_o$. 
%Nevertheless, this issue can be resolved by using predicate pushdown to infer lineage.

% Assuming $Op_i$ is such an operator, when running the pipeline using the lineage rows, we apply the predicate $F_i$ (which is the same as $G_{i+1}$) to the result of $Op_i$. This process ensures that only the precise lineage for the next operator $Op_{i+1}$ is obtained, discarding any extraneous rows.
% However, since this relaxed lineage model is not transitive, computing the pipeline lineage using this model does not guarantee the production of the output $t_o$. However, this can be resolved using predicate pushdown to infer lineage. Assume $Op_i$ is such an operator when running the pipeline using the lineage rows, we apply the predicate $F_i$ (which is the same as $G_{i+1}$) on the result of $Op_i$ such that only the precise lineage for the next operator $Op_{i+1}$ is kept, throwing away extraneous rows.
% The lineage for the data pipeline remains unchanged even when these operators are included, as it is the best effort to include relevant rows affecting the output $t_o$,
% Since such a relaxed lineage model is not transitive, computing the pipeline using the lineage is not guaranteed to produce the output $t_o$. 


% \revised{
% When pushing down predicates, we allow superset when pushing a row-selection predicate $F^{row}$, i.e., retain the most selective $G^{row}$ as long as $Op(G^{row}(T))\supseteq F^{row}(Op(T))$. The rest process remains the same. 
% }
% \yin{superset is confusing, it is not a superset of T* as in Section 6}


%Assuming $Op_i$ is such an operator, when running the pipeline using lineage rows, we apply the predicate $F_i$ (equivalent to $G_{i+1}$) to $Op_i$'s result. This process ensures obtaining only the precise lineage for the next operator $Op_{i+1}$ by discarding extraneous rows. Therefore, when pushing a row-selection predicate $F^{row}$, we enable the return of the most selective $G^{row}$ such that $Op(G^{row}(T))\supseteq F^{row}(Op(T))$. The rest of the process remains unchanged, maintaining the return of precise lineage.


\vspace{-3mm}
\subsection{Scope and limitations}


\textbf{Set semantics.} Because \tool relies on the row-selection predicate to identify the target output, it would track all rows with the same value indistinguishably and return their lineage altogether. 
In our evaluation, because each table/dataframe has a unique index by default, so they inherently follow set semantics.
Given a pipeline, we may be able to add a primary key properly to make every output row at each step distinguishable. We leave it as future work. 
%However, we might be able to add an ``id'' field in each table and slightly modify the pipeline (e.g., including ``id''s during projection) to make each output row at each step distinguishable. We leave it as future work.



\textbf{Scope of UDF supported.} \tool can support UDF embedded in an operator (e.g., user-defined aggregation in groupby) as described in Table~\ref{tab:basic-ops}, but not arbitrary user-defined operators. This is mainly capped by the UDF supported by the predicate pushdown module~\cite{predicate-pushdown}, which requires the UDF to be 1) deterministic, 2) can be symbolically executed \cite{veanes2009symbolic}, 3) cannot allow library functions when embedded in certain operators. As \tool heavily relies on the SMT solver, for complex UDF verification it may incur high overhead or even timeout. However, the verification all finishes within a reasonable time in our evaluation as the UDFs used in open-source data pipelines are relatively simple. 






%\textbf{\tool's lineage model vs. prior work.} We use the same lineage model as Ikeda et. al~\cite{ikeda2013logical}, which slightly differs from other works in certain operators. For example, a {\it GroupBy} operator with {\it max} aggregation, the minimum subset is the row with the max value, while some prior works may include entire group\cite{cui2003lineage,psallidas2018smoke}. \tool can adapted to return the entire group by replacing a predicate pushdown module with one that always returns a $G^{row}$ selecting the entire group.

%\textbf{When pushdown fails.} When pushing an arbitrary predicate fails, \tool falls back to pushing down a row-selection predicate $F^{row}$, and we assume the external pushdown module can always find the most selective predicate for $F^{row}$. This can be easily achieved by MagicPush and other state-of-the-art query optimizers as $F^{row}$ is a special predicate conjuncting equal comparisons. 
%Yet in principle, it may fail. To handle such failure, \tool includes a list of $G^{row}$s for each of the supported operators as shown in Table~\ref{tab:basic-ops}, and returns a pre-defined $G^{row}$.

\begin{comment}
\tool uses SMT solver to find counterexample $r'$ that demonstrates that a pushed predicate $G$ is not minimal, i.e., removing $r'$ from $G(T)$ still produces the target output $t_o$. If such $r'$ cannot be found, we can decide that $G$ selects the minimal subset. 

We explain how the SMT solver works using Q4. 
When pushing down the original predicate $F_4:$ \dbfield{o\_orderpriority}=$v_g$ through the semijoin ($Op_4$), the returned $G$ on table \dbtable{lineitem} selecting all rows, encompassing the lineage as a superset. 

We first construct symbolic tables, which contain symbols to represent cell values, as shown in Figure \ref{fig:counter-ex-minimal}(1). We create two symblic rows for each table, but show only one for the \dbtable{orders} table to simplify explanation. 
Because we use symbols like $v_1$ but not concrete values as table fields, whether the row from \dbtable{orders} will appear in the output depends on the values of $v_2,v_3$ and $v_4$. Therefore we use an indicator {\it row-exist}, which is an expression, to signify whether this row is present in the output or not (as illustrated in Figure~\ref{fig:counter-ex-minimal}(2)). 
%When {\it row-exist} evaluates to \textit{True}, it indicates the presence of the corresponding row.

Pushing down $F_4$ returns $G1:$ \dbfield{o\_orderpriority}\\==$v_g$ on \dbtable{orders} and $G2$: \textit{True} on \dbtable{lineitem}. We set $r'$ as the second row from \dbtable{lineitem} and see if removing $r'$ can still produce an output containing $t_o$. Similarly, we execute $Op(G1(T1), G2(T2)-\{r'\})$ on the symbolic tables and obtain the result as shown in Figure~\ref{fig:counter-ex-minimal}(3). Then we use the SMT solver to solve if such $r'$ can possibly exist, and the solver returns a concrete example of such $r'$, which has a different value of \dbfield{l\_orderkey} ($v_4=2$) than the orders appear in the output ($v_1=1$). As a result, \tool decides that the pushdown returns a lineage superset, and consequently $Op_4$'s output needs to be saved. 
\end{comment}




==> motivation.tex <==
\section{Motivation}
\cong{we can merge this example and workflow.}
\yin{Sure, I will do that.}
%In this section, we present several examples that are commonly seen in real-world pipelines but are not handled by existing lineage systems and algorithms. We demonstrate the challenges of tracing lineage for a wider range of SQL queries, non-relational operators, UDFs, and pipelines that include conditions and branches.
% Panda system \cite{} is a 
% Still many cases and scenarios cannot be handled by the existing work.
% \yin{Give a brief definition of data lineage. The formal ones will be formally discussed in xxx.}

%\textbf{Case study 1: Nested Queries.} 
While existing lineage tracing algorithms have been extensively studied for relational queries, there are still limitations on the type of queries they can handle. For example, nested queries (TPC-H Q2, 4, 17, 18, 20, 21, 22) are not supported by the state-of-the-art lazy lineage inference systems \cite{ikeda2013logical, psallidas2018smoke}. In this case study, we will examine an example of such queries, TPC-H Q4.
%to see how predicate pushdown could trace the data lineage efficiently for nested queries.

\vspace{2mm}
\noindent
\texttt{SELECT }\textit{o\_orderpriority, count(*) as order\_count} \\
\hspace*{1em}\texttt{FROM} \textit{orders} \\
\hspace*{0.5em}\texttt{WHERE} \textit{o\_orderdate > `1993-07-01'} \texttt{AND} \textit{o\_orderdate < `1993-10-01'}\\
% \hspace*{1.5em}\texttt{AND} \textit{o_orderdate < '1993-10-01'}\\
\hspace*{1.5em}\texttt{AND} \texttt{exists(}\\
\hspace*{3em}\texttt{SELECT *} \\
\hspace*{4em}\texttt{FROM} \textit{lineitem}\\
\hspace*{3.5em}\texttt{WHERE} \textit{l\_orderkey = o\_orderkey} \\
\hspace*{4.5em}\texttt{AND} \textit{l\_commitdate < l\_receiptdate})\\
\hspace*{1em}\texttt{GROUP BY} \textit{o\_orderpriority} \\
\hspace*{1em}\texttt{ORDER BY} \textit{o\_orderpriority}; 
\vspace{2mm}

% what traditional method could do and its drawbacks
Given the query above, suppose the data analyst would like to trace the lineage of the output record $t_0$, obtained by a row-selection predicate (\textit{o\_orderpriority} = `1-URGENT' and \textit{order\_count} = 10504). For the \textit{lineitem} table, one could include the records satisfying the predicate in the inner query (\textit{l\_commitdate < l\_receiptdate}) as the lineage set of $t_0$. However, only the records from \textit{lineitems} that could join with the lineage set of $orders$ table are origins of $t_0$. In this example. not all records from the $orders$ table are included in the final result. Therefore, if we only consider the predicates in the inner query, we will obtain a lineage superset. Obtaining the minimal lineage set for the inner table in a nested query has not been previously discussed in prior works.


% In this paper, we study the problem of where-provenance \cite{}, which is an important problem to obtain the source of the output data items. We use a search-verification approach to get the pushdown predicate and use execution snapshots to guarantee the minimality of the lineage set. 
% Our method allows us to study data lineage for more complex queries and non-relation scenarios without using annotations which might slow-down the data loading and refresh. 


\begin{comment}
\textbf{Case study 2: Non-relational operators.} Figure \ref{} shows the example of the 
(use the pipeline 3742233)


(use the pipeline 4264471)

\textbf{Case study 3: Conditions and branches.}


(pipeline 455979)
(pipeline 4463564)

\paragraph{Non-relational operators}
1. unpivot
2. set item (attribute mapping containing functions (domain changes))


lacks a  xxx to determine when 

\paragraph{Data pipeline containing conditions and branches}

if condition

\textbf{Case study 4: Augmentation and Snapshots.}
\end{comment}
